The Twins Embedding of Type Ia Supernovae I: The Diversity of Spectra at Maximum Light

We study the spectral diversity of Type Ia supernovae (SNe Ia) at maximum light using high signal-to-noise spectrophotometry of 173 SNe Ia from the Nearby Supernova Factory. We decompose the diversity of these spectra into different extrinsic and intrinsic components, and we construct a nonlinear parameterization of the intrinsic diversity of SNe Ia that preserves pairings of "twin" SNe Ia. We call this parameterization the "Twins Embedding". Our methodology naturally handles highly nonlinear variability in spectra, such as changes in the photosphere expansion velocity, and uses the full spectrum rather than being limited to specific spectral line strengths, ratios or velocities. We find that the time evolution of SNe Ia near maximum light is remarkably similar, with 84.6% of the variance in common to all SNe Ia. After correcting for brightness and color, the intrinsic variability of SNe Ia is mostly restricted to specific spectral lines, and we find intrinsic dispersions as low as ~0.02 mag between 6600 and 7200 A. With a nonlinear three-dimensional model plus one dimension for color, we can explain 89.2% of the intrinsic diversity in our sample of SNe Ia, which includes several different kinds of "peculiar" SNe Ia. A linear model requires seven dimensions to explain a comparable fraction of the intrinsic diversity. We show how a wide range of previously-established indicators of diversity in SNe Ia can be recovered from the Twins Embedding. In a companion article, we discuss how these results an be applied to standardization of SNe Ia for cosmology.

==> latex/differential_time_evolution_parameters.tex <==
3305 & 0.112 & 0.00845 & 0.154 & 0.033 & 0.108 & 0.134 & 0.247 \\
3316 & 0.115 & 0.00860 & 0.152 & 0.029 & 0.128 & 0.149 & 0.262 \\
3327 & 0.118 & 0.00893 & 0.157 & 0.021 & 0.119 & 0.137 & 0.269 \\
3338 & 0.116 & 0.00999 & 0.131 & 0.030 & 0.123 & 0.142 & 0.278 \\
3349 & 0.114 & 0.01013 & 0.121 & 0.038 & 0.113 & 0.131 & 0.270 \\
3360 & 0.111 & 0.01024 & 0.139 & 0.021 & 0.110 & 0.132 & 0.245 \\
3372 & 0.106 & 0.00993 & 0.124 & 0.021 & 0.092 & 0.112 & 0.227 \\
3383 & 0.103 & 0.00954 & 0.113 & 0.021 & 0.094 & 0.116 & 0.219 \\
3394 & 0.102 & 0.00948 & 0.125 & 0.015 & 0.085 & 0.099 & 0.208 \\
3405 & 0.103 & 0.00965 & 0.139 & 0.015 & 0.068 & 0.084 & 0.201 \\
3417 & 0.104 & 0.00924 & 0.125 & 0.012 & 0.071 & 0.083 & 0.198 \\
3428 & 0.108 & 0.00953 & 0.098 & 0.014 & 0.073 & 0.087 & 0.193 \\
3440 & 0.110 & 0.00982 & 0.078 & 0.015 & 0.068 & 0.084 & 0.189 \\
3451 & 0.108 & 0.01096 & 0.058 & 0.024 & 0.063 & 0.083 & 0.177 \\
3463 & 0.102 & 0.01134 & 0.061 & 0.024 & 0.062 & 0.083 & 0.160 \\
3474 & 0.093 & 0.01148 & 0.072 & 0.024 & 0.066 & 0.088 & 0.138 \\
3486 & 0.086 & 0.01168 & 0.045 & 0.027 & 0.066 & 0.096 & 0.123 \\
3497 & 0.076 & 0.01113 & 0.041 & 0.030 & 0.067 & 0.098 & 0.119 \\
3509 & 0.065 & 0.01104 & 0.048 & 0.026 & 0.072 & 0.109 & 0.114 \\
3521 & 0.053 & 0.01022 & 0.047 & 0.020 & 0.081 & 0.104 & 0.114 \\
3532 & 0.048 & 0.01031 & 0.049 & 0.026 & 0.075 & 0.109 & 0.117 \\
3544 & 0.043 & 0.01030 & 0.049 & 0.026 & 0.070 & 0.123 & 0.124 \\
3556 & 0.038 & 0.01052 & 0.070 & 0.025 & 0.062 & 0.123 & 0.138 \\
3568 & 0.035 & 0.01070 & 0.100 & 0.026 & 0.053 & 0.122 & 0.155 \\
3580 & 0.030 & 0.01201 & 0.146 & 0.029 & 0.059 & 0.118 & 0.173 \\
3592 & 0.024 & 0.01366 & 0.221 & 0.039 & 0.062 & 0.135 & 0.188 \\
3604 & 0.018 & 0.01478 & 0.269 & 0.073 & 0.061 & 0.165 & 0.207 \\
3616 & 0.010 & 0.01551 & 0.311 & 0.085 & 0.071 & 0.191 & 0.230 \\
3628 & -0.003 & 0.01717 & 0.349 & 0.105 & 0.089 & 0.221 & 0.257 \\
3640 & -0.013 & 0.01640 & 0.302 & 0.115 & 0.087 & 0.248 & 0.293 \\
3652 & -0.018 & 0.01348 & 0.231 & 0.085 & 0.093 & 0.252 & 0.348 \\
3664 & -0.016 & 0.01072 & 0.189 & 0.040 & 0.116 & 0.213 & 0.401 \\
3676 & -0.018 & 0.00906 & 0.175 & 0.055 & 0.064 & 0.190 & 0.430 \\
3688 & -0.010 & 0.00777 & 0.128 & 0.051 & 0.050 & 0.178 & 0.451 \\
3701 & 0.002 & 0.00732 & 0.125 & 0.069 & 0.037 & 0.173 & 0.440 \\
3713 & 0.013 & 0.00599 & 0.118 & 0.058 & 0.044 & 0.145 & 0.420 \\
3725 & 0.026 & 0.00534 & 0.101 & 0.059 & 0.037 & 0.137 & 0.404 \\
3738 & 0.038 & 0.00481 & 0.107 & 0.042 & 0.046 & 0.118 & 0.392 \\
3750 & 0.046 & 0.00547 & 0.086 & 0.022 & 0.056 & 0.105 & 0.381 \\
3763 & 0.050 & 0.00605 & 0.085 & 0.016 & 0.057 & 0.092 & 0.346 \\
3775 & 0.050 & 0.00606 & 0.075 & 0.040 & 0.027 & 0.092 & 0.321 \\
3788 & 0.049 & 0.00590 & 0.074 & 0.020 & 0.035 & 0.091 & 0.284 \\
3801 & 0.049 & 0.00577 & 0.069 & 0.023 & 0.035 & 0.095 & 0.246 \\
3813 & 0.046 & 0.00489 & 0.071 & 0.014 & 0.045 & 0.088 & 0.198 \\
3826 & 0.045 & 0.00492 & 0.060 & 0.018 & 0.047 & 0.099 & 0.164 \\
3839 & 0.042 & 0.00583 & 0.040 & 0.014 & 0.046 & 0.096 & 0.133 \\
3851 & 0.037 & 0.00780 & 0.040 & 0.026 & 0.041 & 0.106 & 0.100 \\
3864 & 0.024 & 0.00816 & 0.030 & 0.021 & 0.049 & 0.103 & 0.080 \\
3877 & 0.013 & 0.00745 & 0.027 & 0.014 & 0.062 & 0.105 & 0.076 \\
3890 & 0.009 & 0.00691 & 0.039 & 0.014 & 0.054 & 0.108 & 0.079 \\
3903 & 0.010 & 0.00633 & 0.048 & 0.025 & 0.048 & 0.097 & 0.078 \\
3916 & 0.014 & 0.00629 & 0.040 & 0.019 & 0.044 & 0.097 & 0.072 \\
3929 & 0.016 & 0.00673 & 0.040 & 0.018 & 0.037 & 0.089 & 0.078 \\
3942 & 0.014 & 0.00729 & 0.051 & 0.017 & 0.043 & 0.082 & 0.086 \\
3955 & 0.013 & 0.00739 & 0.066 & 0.027 & 0.030 & 0.076 & 0.092 \\
3968 & 0.017 & 0.00738 & 0.068 & 0.031 & 0.040 & 0.081 & 0.084 \\
3982 & 0.022 & 0.00800 & 0.060 & 0.030 & 0.032 & 0.081 & 0.076 \\
3995 & 0.027 & 0.00910 & 0.039 & 0.025 & 0.030 & 0.081 & 0.074 \\
4008 & 0.026 & 0.00904 & 0.023 & 0.012 & 0.058 & 0.074 & 0.079 \\
4022 & 0.026 & 0.00930 & 0.026 & 0.016 & 0.048 & 0.076 & 0.080 \\
4035 & 0.023 & 0.00928 & 0.026 & 0.013 & 0.049 & 0.086 & 0.068 \\
4048 & 0.019 & 0.00892 & 0.021 & 0.011 & 0.055 & 0.089 & 0.063 \\
4062 & 0.018 & 0.00898 & 0.023 & 0.011 & 0.054 & 0.095 & 0.066 \\
4075 & 0.018 & 0.00902 & 0.023 & 0.008 & 0.062 & 0.101 & 0.070 \\
4089 & 0.018 & 0.00876 & 0.023 & 0.007 & 0.056 & 0.111 & 0.080 \\
4103 & 0.017 & 0.00929 & 0.044 & 0.014 & 0.044 & 0.115 & 0.093 \\
4116 & 0.015 & 0.00937 & 0.064 & 0.028 & 0.033 & 0.117 & 0.096 \\
4130 & 0.015 & 0.00928 & 0.053 & 0.038 & 0.026 & 0.128 & 0.090 \\
4144 & 0.013 & 0.00981 & 0.035 & 0.028 & 0.042 & 0.114 & 0.076 \\
4158 & 0.007 & 0.00959 & 0.021 & 0.013 & 0.064 & 0.111 & 0.067 \\
4171 & -0.001 & 0.00944 & 0.035 & 0.011 & 0.059 & 0.120 & 0.072 \\
4185 & -0.007 & 0.00866 & 0.033 & 0.014 & 0.047 & 0.126 & 0.082 \\
4199 & -0.009 & 0.00793 & 0.034 & 0.006 & 0.054 & 0.119 & 0.092 \\
4213 & -0.010 & 0.00759 & 0.032 & 0.006 & 0.058 & 0.121 & 0.092 \\
4227 & -0.009 & 0.00739 & 0.029 & 0.005 & 0.054 & 0.117 & 0.094 \\
4241 & -0.009 & 0.00699 & 0.036 & 0.005 & 0.052 & 0.113 & 0.097 \\
4256 & -0.008 & 0.00618 & 0.047 & 0.019 & 0.034 & 0.111 & 0.104 \\
4270 & -0.006 & 0.00580 & 0.067 & 0.029 & 0.021 & 0.100 & 0.103 \\
4284 & 0.002 & 0.00541 & 0.072 & 0.035 & 0.027 & 0.081 & 0.078 \\
4298 & 0.012 & 0.00523 & 0.059 & 0.027 & 0.035 & 0.084 & 0.058 \\
4313 & 0.020 & 0.00592 & 0.056 & 0.022 & 0.032 & 0.083 & 0.066 \\
4327 & 0.026 & 0.00635 & 0.072 & 0.013 & 0.041 & 0.070 & 0.074 \\
4341 & 0.031 & 0.00673 & 0.063 & 0.016 & 0.040 & 0.074 & 0.069 \\
4356 & 0.034 & 0.00817 & 0.055 & 0.009 & 0.043 & 0.083 & 0.065 \\
4370 & 0.032 & 0.00998 & 0.079 & 0.029 & 0.028 & 0.075 & 0.066 \\
4385 & 0.023 & 0.01182 & 0.086 & 0.051 & 0.032 & 0.088 & 0.064 \\
4400 & 0.008 & 0.01171 & 0.068 & 0.047 & 0.055 & 0.117 & 0.059 \\
4414 & -0.001 & 0.00928 & 0.048 & 0.039 & 0.066 & 0.124 & 0.067 \\
4429 & -0.001 & 0.00693 & 0.041 & 0.031 & 0.054 & 0.129 & 0.079 \\
4444 & 0.004 & 0.00625 & 0.044 & 0.031 & 0.040 & 0.120 & 0.084 \\
4458 & 0.006 & 0.00679 & 0.041 & 0.032 & 0.037 & 0.108 & 0.071 \\
4473 & 0.003 & 0.00772 & 0.035 & 0.028 & 0.043 & 0.110 & 0.064 \\
4488 & -0.002 & 0.00742 & 0.026 & 0.021 & 0.042 & 0.114 & 0.064 \\
4503 & -0.004 & 0.00674 & 0.019 & 0.015 & 0.039 & 0.118 & 0.072 \\
4518 & -0.006 & 0.00626 & 0.039 & 0.006 & 0.037 & 0.112 & 0.076 \\
4533 & -0.007 & 0.00551 & 0.057 & 0.021 & 0.023 & 0.099 & 0.082 \\
4548 & -0.005 & 0.00570 & 0.055 & 0.021 & 0.028 & 0.071 & 0.080 \\
4563 & -0.002 & 0.00609 & 0.056 & 0.020 & 0.023 & 0.060 & 0.075 \\
4579 & -0.004 & 0.00695 & 0.037 & 0.009 & 0.027 & 0.061 & 0.066 \\
4594 & -0.007 & 0.00688 & 0.037 & 0.005 & 0.025 & 0.054 & 0.066 \\
4609 & -0.012 & 0.00669 & 0.039 & 0.008 & 0.021 & 0.046 & 0.073 \\
4625 & -0.015 & 0.00658 & 0.038 & 0.005 & 0.019 & 0.038 & 0.085 \\
4640 & -0.016 & 0.00639 & 0.025 & 0.009 & 0.022 & 0.045 & 0.091 \\
4655 & -0.011 & 0.00564 & 0.019 & 0.006 & 0.029 & 0.051 & 0.087 \\
4671 & -0.004 & 0.00587 & 0.021 & 0.004 & 0.029 & 0.058 & 0.076 \\
4687 & 0.000 & 0.00655 & 0.023 & 0.003 & 0.026 & 0.063 & 0.070 \\
4702 & 0.003 & 0.00750 & 0.034 & 0.006 & 0.023 & 0.057 & 0.072 \\
4718 & 0.003 & 0.00809 & 0.048 & 0.008 & 0.026 & 0.072 & 0.079 \\
4734 & 0.004 & 0.00719 & 0.040 & 0.010 & 0.023 & 0.069 & 0.083 \\
4749 & 0.009 & 0.00689 & 0.030 & 0.007 & 0.029 & 0.051 & 0.076 \\
4765 & 0.013 & 0.00672 & 0.039 & 0.007 & 0.029 & 0.042 & 0.080 \\
4781 & 0.012 & 0.00698 & 0.042 & 0.020 & 0.019 & 0.041 & 0.085 \\
4797 & 0.008 & 0.00759 & 0.041 & 0.009 & 0.028 & 0.050 & 0.095 \\
4813 & 0.004 & 0.00772 & 0.043 & 0.011 & 0.026 & 0.070 & 0.110 \\
4829 & -0.000 & 0.00754 & 0.050 & 0.023 & 0.023 & 0.073 & 0.122 \\
4845 & -0.002 & 0.00693 & 0.062 & 0.016 & 0.036 & 0.070 & 0.119 \\
4861 & -0.003 & 0.00590 & 0.075 & 0.037 & 0.031 & 0.067 & 0.123 \\
4877 & -0.007 & 0.00526 & 0.061 & 0.035 & 0.034 & 0.058 & 0.117 \\
4894 & -0.012 & 0.00520 & 0.049 & 0.015 & 0.039 & 0.052 & 0.087 \\
4910 & -0.012 & 0.00472 & 0.023 & 0.005 & 0.033 & 0.045 & 0.066 \\
4926 & -0.008 & 0.00474 & 0.024 & 0.013 & 0.037 & 0.047 & 0.067 \\
4943 & -0.002 & 0.00577 & 0.040 & 0.015 & 0.040 & 0.060 & 0.077 \\
4959 & 0.003 & 0.00638 & 0.054 & 0.029 & 0.042 & 0.063 & 0.083 \\
4976 & 0.009 & 0.00652 & 0.054 & 0.030 & 0.036 & 0.048 & 0.070 \\
4992 & 0.013 & 0.00640 & 0.055 & 0.024 & 0.031 & 0.042 & 0.059 \\
5009 & 0.015 & 0.00631 & 0.061 & 0.026 & 0.031 & 0.039 & 0.050 \\
5026 & 0.014 & 0.00683 & 0.047 & 0.024 & 0.041 & 0.052 & 0.049 \\
5042 & 0.013 & 0.00739 & 0.039 & 0.019 & 0.035 & 0.044 & 0.048 \\
5059 & 0.009 & 0.00773 & 0.033 & 0.014 & 0.038 & 0.048 & 0.058 \\
5076 & 0.004 & 0.00790 & 0.021 & 0.007 & 0.041 & 0.054 & 0.055 \\
5093 & -0.003 & 0.00799 & 0.022 & 0.006 & 0.052 & 0.062 & 0.056 \\
5110 & -0.010 & 0.00771 & 0.029 & 0.019 & 0.030 & 0.060 & 0.055 \\
5127 & -0.017 & 0.00677 & 0.026 & 0.015 & 0.040 & 0.071 & 0.053 \\
5144 & -0.018 & 0.00611 & 0.028 & 0.015 & 0.043 & 0.070 & 0.053 \\
5161 & -0.017 & 0.00545 & 0.036 & 0.016 & 0.036 & 0.080 & 0.049 \\
5178 & -0.017 & 0.00550 & 0.047 & 0.015 & 0.035 & 0.087 & 0.045 \\
5196 & -0.020 & 0.00569 & 0.052 & 0.022 & 0.035 & 0.098 & 0.050 \\
5213 & -0.027 & 0.00536 & 0.061 & 0.013 & 0.052 & 0.089 & 0.080 \\
5230 & -0.033 & 0.00422 & 0.069 & 0.030 & 0.026 & 0.084 & 0.105 \\
5248 & -0.032 & 0.00319 & 0.076 & 0.046 & 0.025 & 0.102 & 0.119 \\
5265 & -0.025 & 0.00310 & 0.074 & 0.053 & 0.030 & 0.100 & 0.109 \\
5283 & -0.016 & 0.00248 & 0.054 & 0.040 & 0.039 & 0.096 & 0.098 \\
5300 & -0.013 & 0.00259 & 0.035 & 0.022 & 0.047 & 0.081 & 0.084 \\
5318 & -0.009 & 0.00294 & 0.041 & 0.023 & 0.038 & 0.084 & 0.076 \\
5336 & -0.006 & 0.00390 & 0.033 & 0.013 & 0.048 & 0.074 & 0.059 \\
5353 & -0.008 & 0.00510 & 0.035 & 0.020 & 0.025 & 0.069 & 0.047 \\
5371 & -0.013 & 0.00513 & 0.043 & 0.022 & 0.022 & 0.059 & 0.044 \\
5389 & -0.017 & 0.00536 & 0.045 & 0.013 & 0.040 & 0.066 & 0.056 \\
5407 & -0.021 & 0.00455 & 0.054 & 0.009 & 0.088 & 0.093 & 0.070 \\
5425 & -0.021 & 0.00393 & 0.058 & 0.030 & 0.030 & 0.056 & 0.084 \\
5443 & -0.015 & 0.00289 & 0.067 & 0.051 & 0.011 & 0.082 & 0.104 \\
5461 & -0.003 & 0.00326 & 0.042 & 0.026 & 0.050 & 0.079 & 0.128 \\
5480 & 0.002 & 0.00381 & 0.040 & 0.029 & 0.044 & 0.069 & 0.136 \\
5498 & 0.001 & 0.00483 & 0.038 & 0.020 & 0.041 & 0.064 & 0.116 \\
5516 & -0.003 & 0.00601 & 0.055 & 0.008 & 0.044 & 0.056 & 0.089 \\
5534 & -0.014 & 0.00696 & 0.046 & 0.035 & 0.019 & 0.034 & 0.074 \\
5553 & -0.021 & 0.00795 & 0.028 & 0.023 & 0.025 & 0.044 & 0.060 \\
5571 & -0.025 & 0.00715 & 0.023 & 0.016 & 0.029 & 0.053 & 0.063 \\
5590 & -0.026 & 0.00705 & 0.032 & 0.009 & 0.033 & 0.058 & 0.062 \\
5609 & -0.025 & 0.00635 & 0.020 & 0.010 & 0.027 & 0.055 & 0.059 \\
5627 & -0.023 & 0.00575 & 0.016 & 0.011 & 0.027 & 0.051 & 0.059 \\
5646 & -0.019 & 0.00601 & 0.024 & 0.015 & 0.025 & 0.043 & 0.057 \\
5665 & -0.016 & 0.00647 & 0.026 & 0.018 & 0.021 & 0.041 & 0.058 \\
5684 & -0.014 & 0.00748 & 0.035 & 0.018 & 0.017 & 0.042 & 0.062 \\
5703 & -0.015 & 0.00814 & 0.050 & 0.026 & 0.014 & 0.040 & 0.068 \\
5722 & -0.017 & 0.00780 & 0.046 & 0.032 & 0.014 & 0.042 & 0.086 \\
5741 & -0.017 & 0.00733 & 0.037 & 0.028 & 0.017 & 0.045 & 0.110 \\
5760 & -0.015 & 0.00656 & 0.030 & 0.018 & 0.014 & 0.036 & 0.127 \\
5779 & -0.015 & 0.00619 & 0.027 & 0.014 & 0.006 & 0.027 & 0.130 \\
5798 & -0.017 & 0.00642 & 0.028 & 0.016 & 0.006 & 0.026 & 0.117 \\
5818 & -0.021 & 0.00611 & 0.031 & 0.019 & 0.010 & 0.023 & 0.098 \\
5837 & -0.022 & 0.00543 & 0.025 & 0.018 & 0.008 & 0.029 & 0.080 \\
5856 & -0.022 & 0.00494 & 0.024 & 0.019 & 0.009 & 0.027 & 0.064 \\
5876 & -0.019 & 0.00518 & 0.029 & 0.013 & 0.007 & 0.038 & 0.054 \\
5896 & -0.019 & 0.00610 & 0.047 & 0.017 & 0.008 & 0.044 & 0.059 \\
5915 & -0.020 & 0.00681 & 0.071 & 0.016 & 0.016 & 0.039 & 0.055 \\
5935 & -0.021 & 0.00691 & 0.076 & 0.023 & 0.018 & 0.042 & 0.065 \\
5955 & -0.021 & 0.00772 & 0.074 & 0.026 & 0.016 & 0.057 & 0.081 \\
5975 & -0.024 & 0.00829 & 0.071 & 0.029 & 0.017 & 0.054 & 0.104 \\
5994 & -0.025 & 0.00849 & 0.074 & 0.026 & 0.018 & 0.057 & 0.133 \\
6014 & -0.028 & 0.00838 & 0.081 & 0.033 & 0.019 & 0.050 & 0.166 \\
6034 & -0.029 & 0.00811 & 0.091 & 0.046 & 0.022 & 0.072 & 0.208 \\
6055 & -0.024 & 0.00686 & 0.092 & 0.042 & 0.033 & 0.084 & 0.252 \\
6075 & -0.013 & 0.00643 & 0.101 & 0.047 & 0.038 & 0.086 & 0.287 \\
6095 & 0.003 & 0.00552 & 0.073 & 0.043 & 0.040 & 0.075 & 0.301 \\
6115 & 0.013 & 0.00467 & 0.049 & 0.035 & 0.039 & 0.081 & 0.294 \\
6136 & 0.019 & 0.00482 & 0.067 & 0.030 & 0.041 & 0.091 & 0.276 \\
6156 & 0.018 & 0.00440 & 0.073 & 0.032 & 0.042 & 0.071 & 0.251 \\
6177 & 0.012 & 0.00388 & 0.082 & 0.037 & 0.035 & 0.059 & 0.214 \\
6197 & 0.003 & 0.00459 & 0.076 & 0.031 & 0.030 & 0.057 & 0.167 \\
6218 & -0.006 & 0.00522 & 0.069 & 0.032 & 0.019 & 0.036 & 0.123 \\
6239 & -0.011 & 0.00547 & 0.045 & 0.026 & 0.011 & 0.026 & 0.090 \\
6259 & -0.012 & 0.00535 & 0.035 & 0.016 & 0.008 & 0.027 & 0.072 \\
6280 & -0.013 & 0.00552 & 0.027 & 0.009 & 0.011 & 0.024 & 0.065 \\
6301 & -0.013 & 0.00583 & 0.025 & 0.014 & 0.009 & 0.026 & 0.062 \\
6322 & -0.014 & 0.00605 & 0.029 & 0.018 & 0.010 & 0.021 & 0.066 \\
6343 & -0.015 & 0.00607 & 0.032 & 0.021 & 0.013 & 0.018 & 0.067 \\
6364 & -0.014 & 0.00560 & 0.028 & 0.018 & 0.012 & 0.024 & 0.071 \\
6385 & -0.014 & 0.00542 & 0.024 & 0.019 & 0.013 & 0.023 & 0.072 \\
6407 & -0.015 & 0.00514 & 0.028 & 0.020 & 0.008 & 0.024 & 0.068 \\
6428 & -0.016 & 0.00485 & 0.025 & 0.019 & 0.013 & 0.021 & 0.063 \\
6449 & -0.016 & 0.00452 & 0.028 & 0.017 & 0.015 & 0.023 & 0.057 \\
6471 & -0.017 & 0.00441 & 0.027 & 0.015 & 0.011 & 0.021 & 0.052 \\
6493 & -0.017 & 0.00384 & 0.030 & 0.019 & 0.011 & 0.023 & 0.047 \\
6514 & -0.016 & 0.00368 & 0.032 & 0.023 & 0.008 & 0.022 & 0.040 \\
6536 & -0.017 & 0.00384 & 0.036 & 0.017 & 0.013 & 0.022 & 0.035 \\
6558 & -0.016 & 0.00376 & 0.049 & 0.021 & 0.010 & 0.023 & 0.033 \\
6579 & -0.016 & 0.00356 & 0.050 & 0.020 & 0.010 & 0.019 & 0.027 \\
6601 & -0.014 & 0.00330 & 0.047 & 0.025 & 0.010 & 0.017 & 0.026 \\
6623 & -0.012 & 0.00298 & 0.046 & 0.019 & 0.010 & 0.019 & 0.024 \\
6645 & -0.011 & 0.00337 & 0.062 & 0.026 & 0.007 & 0.017 & 0.019 \\
6668 & -0.010 & 0.00329 & 0.059 & 0.031 & 0.006 & 0.021 & 0.019 \\
6690 & -0.011 & 0.00343 & 0.072 & 0.033 & 0.007 & 0.022 & 0.020 \\
6712 & -0.010 & 0.00289 & 0.056 & 0.034 & 0.009 & 0.022 & 0.017 \\
6734 & -0.009 & 0.00239 & 0.064 & 0.032 & 0.008 & 0.021 & 0.017 \\
6757 & -0.008 & 0.00204 & 0.077 & 0.033 & 0.008 & 0.017 & 0.019 \\
6779 & -0.008 & 0.00189 & 0.077 & 0.042 & 0.005 & 0.018 & 0.023 \\
6802 & -0.007 & 0.00153 & 0.070 & 0.040 & 0.006 & 0.018 & 0.026 \\
6825 & -0.005 & 0.00104 & 0.075 & 0.038 & 0.010 & 0.026 & 0.024 \\
6847 & -0.004 & 0.00093 & 0.066 & 0.035 & 0.007 & 0.019 & 0.017 \\
6870 & -0.002 & 0.00066 & 0.061 & 0.037 & 0.007 & 0.025 & 0.017 \\
6893 & 0.000 & 0.00046 & 0.067 & 0.041 & 0.005 & 0.023 & 0.016 \\
6916 & 0.004 & 0.00073 & 0.061 & 0.038 & 0.003 & 0.019 & 0.014 \\
6939 & 0.006 & 0.00088 & 0.055 & 0.043 & 0.005 & 0.022 & 0.016 \\
6962 & 0.009 & 0.00062 & 0.051 & 0.035 & 0.008 & 0.019 & 0.013 \\
6985 & 0.010 & 0.00057 & 0.053 & 0.035 & 0.005 & 0.023 & 0.015 \\
7009 & 0.014 & 0.00023 & 0.061 & 0.029 & 0.009 & 0.017 & 0.018 \\
7032 & 0.016 & 0.00047 & 0.058 & 0.038 & 0.008 & 0.021 & 0.015 \\
7055 & 0.018 & 0.00058 & 0.057 & 0.035 & 0.011 & 0.029 & 0.015 \\
7079 & 0.019 & 0.00070 & 0.056 & 0.036 & 0.008 & 0.019 & 0.022 \\
7103 & 0.019 & 0.00065 & 0.060 & 0.047 & 0.007 & 0.021 & 0.024 \\
7126 & 0.019 & 0.00027 & 0.066 & 0.041 & 0.008 & 0.015 & 0.026 \\
7150 & 0.019 & 0.00004 & 0.067 & 0.040 & 0.010 & 0.019 & 0.027 \\
7174 & 0.019 & 0.00015 & 0.063 & 0.042 & 0.010 & 0.022 & 0.030 \\
7198 & 0.019 & 0.00003 & 0.069 & 0.041 & 0.010 & 0.021 & 0.029 \\
7222 & 0.017 & 0.00014 & 0.066 & 0.046 & 0.010 & 0.019 & 0.030 \\
7246 & 0.016 & 0.00001 & 0.060 & 0.043 & 0.016 & 0.030 & 0.035 \\
7270 & 0.017 & -0.00027 & 0.076 & 0.045 & 0.019 & 0.041 & 0.039 \\
7294 & 0.020 & -0.00046 & 0.075 & 0.046 & 0.022 & 0.039 & 0.047 \\
7318 & 0.025 & -0.00049 & 0.077 & 0.052 & 0.025 & 0.049 & 0.049 \\
7343 & 0.029 & -0.00034 & 0.086 & 0.061 & 0.023 & 0.064 & 0.056 \\
7367 & 0.033 & -0.00049 & 0.086 & 0.061 & 0.025 & 0.074 & 0.062 \\
7392 & 0.038 & 0.00030 & 0.089 & 0.060 & 0.029 & 0.096 & 0.085 \\
7416 & 0.040 & -0.00064 & 0.090 & 0.063 & 0.031 & 0.073 & 0.113 \\
7441 & 0.044 & -0.00081 & 0.092 & 0.066 & 0.031 & 0.073 & 0.133 \\
7466 & 0.050 & -0.00110 & 0.104 & 0.065 & 0.036 & 0.070 & 0.146 \\
7491 & 0.051 & -0.00002 & 0.098 & 0.060 & 0.032 & 0.074 & 0.130 \\
7516 & 0.050 & -0.00000 & 0.096 & 0.069 & 0.023 & 0.061 & 0.110 \\
7541 & 0.046 & 0.00107 & 0.073 & 0.060 & 0.026 & 0.074 & 0.077 \\
7566 & 0.044 & 0.00096 & 0.068 & 0.056 & 0.031 & 0.065 & 0.060 \\
7591 & 0.043 & 0.00160 & 0.059 & 0.046 & 0.035 & 0.068 & 0.052 \\
7616 & 0.042 & 0.00175 & 0.056 & 0.046 & 0.028 & 0.067 & 0.045 \\
7642 & 0.042 & 0.00182 & 0.061 & 0.041 & 0.028 & 0.071 & 0.057 \\
7667 & 0.043 & 0.00198 & 0.061 & 0.040 & 0.026 & 0.078 & 0.070 \\
7693 & 0.043 & 0.00225 & 0.068 & 0.044 & 0.020 & 0.087 & 0.081 \\
7718 & 0.042 & 0.00302 & 0.058 & 0.041 & 0.025 & 0.075 & 0.075 \\
7744 & 0.038 & 0.00335 & 0.053 & 0.037 & 0.025 & 0.070 & 0.079 \\
7770 & 0.035 & 0.00374 & 0.056 & 0.037 & 0.025 & 0.067 & 0.079 \\
7796 & 0.028 & 0.00397 & 0.061 & 0.037 & 0.024 & 0.060 & 0.083 \\
7822 & 0.020 & 0.00453 & 0.067 & 0.038 & 0.025 & 0.062 & 0.082 \\
7848 & 0.012 & 0.00540 & 0.077 & 0.045 & 0.025 & 0.063 & 0.089 \\
7874 & 0.006 & 0.00583 & 0.111 & 0.056 & 0.022 & 0.063 & 0.109 \\
7900 & 0.000 & 0.00628 & 0.116 & 0.061 & 0.027 & 0.067 & 0.123 \\
7927 & -0.000 & 0.00642 & 0.108 & 0.077 & 0.023 & 0.075 & 0.146 \\
7953 & -0.001 & 0.00648 & 0.118 & 0.064 & 0.026 & 0.080 & 0.165 \\
7979 & 0.000 & 0.00670 & 0.100 & 0.066 & 0.023 & 0.081 & 0.181 \\
8006 & 0.003 & 0.00584 & 0.098 & 0.054 & 0.022 & 0.069 & 0.191 \\
8033 & 0.010 & 0.00523 & 0.093 & 0.041 & 0.043 & 0.063 & 0.197 \\
8059 & 0.021 & 0.00480 & 0.074 & 0.054 & 0.033 & 0.076 & 0.209 \\
8086 & 0.030 & 0.00558 & 0.070 & 0.052 & 0.038 & 0.096 & 0.228 \\
8113 & 0.041 & 0.00600 & 0.099 & 0.044 & 0.049 & 0.113 & 0.246 \\
8140 & 0.049 & 0.00674 & 0.095 & 0.057 & 0.031 & 0.126 & 0.273 \\
8167 & 0.056 & 0.00698 & 0.118 & 0.051 & 0.040 & 0.112 & 0.285 \\
8195 & 0.063 & 0.00692 & 0.107 & 0.067 & 0.041 & 0.083 & 0.283 \\
8222 & 0.065 & 0.00716 & 0.101 & 0.041 & 0.038 & 0.105 & 0.261 \\
8249 & 0.065 & 0.00658 & 0.113 & 0.046 & 0.052 & 0.086 & 0.246 \\
8277 & 0.057 & 0.00730 & 0.097 & 0.045 & 0.059 & 0.103 & 0.234 \\
8304 & 0.049 & 0.00652 & 0.105 & 0.055 & 0.043 & 0.105 & 0.212 \\
8332 & 0.042 & 0.00601 & 0.109 & 0.060 & 0.043 & 0.090 & 0.195 \\
8360 & 0.034 & 0.00668 & 0.112 & 0.041 & 0.044 & 0.098 & 0.167 \\
8388 & 0.025 & 0.00591 & 0.105 & 0.049 & 0.035 & 0.099 & 0.135 \\
8416 & 0.014 & 0.00595 & 0.103 & 0.039 & 0.032 & 0.087 & 0.107 \\
8444 & 0.004 & 0.00557 & 0.095 & 0.052 & 0.024 & 0.077 & 0.088 \\
8472 & -0.004 & 0.00519 & 0.068 & 0.044 & 0.021 & 0.048 & 0.066 \\
8500 & -0.009 & 0.00489 & 0.071 & 0.032 & 0.014 & 0.042 & 0.066 \\
8528 & -0.012 & 0.00443 & 0.056 & 0.039 & 0.016 & 0.044 & 0.069 \\
8557 & -0.016 & 0.00470 & 0.057 & 0.028 & 0.016 & 0.037 & 0.074 \\
8585 & -0.018 & 0.00411 & 0.048 & 0.036 & 0.010 & 0.034 & 0.075 \\


==> latex/twins_manifold_coordinates.tex <==
SN2011gf & 0.97 & 0.17 & -0.148 & 0.029 & -0.385 & 0.012 & 0.094 & 0.082 & -0.541 & 0.579 & -1.274 \\
SN2011ga & -0.11 & 0.20 & -0.057 & 0.031 & -0.112 & 0.012 & 0.040 & 0.058 & 0.304 & -0.828 & 0.573 \\
CSS120424\_01 & 0.92 & 0.19 & -0.062 & 0.030 & -0.171 & 0.013 & 0.026 & 0.059 & -1.188 & 1.068 & 0.407 \\
CSS130502\_01 & -0.03 & 0.21 & -0.107 & 0.031 & -0.217 & 0.012 & 0.186 & 0.065 & 2.089 & -1.109 & -0.322 \\
LSQ12dbr & 1.12 & 0.10 & -0.140 & 0.027 & -0.377 & 0.012 & 0.038 & 0.117 & 0.124 & 0.953 & -1.644 \\
LSQ12ekl & -0.65 & 0.13 & -0.074 & 0.029 & 0.139 & 0.016 & -0.043 & 0.033 & 0.321 & -1.589 & 0.983 \\
LSQ12fhe & 1.21 & 0.18 & 0.030 & 0.030 & -0.075 & 0.012 & -0.341 & 0.083 & 4.811 & 1.137 & -0.689 \\
LSQ12fhs & -1.11 & 0.26 & 0.390 & 0.037 & 1.294 & 0.013 & 0.008 & 0.069 & 7.327 & 4.931 & 2.777 \\
LSQ12fxd & 0.31 & 0.14 & -0.049 & 0.030 & -0.154 & 0.012 & -0.183 & 0.070 & -1.082 & 2.327 & 0.288 \\
LSQ12gxj & 0.80 & 0.21 & 0.213 & 0.035 & 0.538 & 0.013 & 0.523 & 0.064 & 0.517 & 0.834 & -1.160 \\
LSQ12hjm & -0.70 & 0.23 & -0.112 & 0.035 & -0.131 & 0.013 & 0.061 & 0.033 & 2.270 & -1.307 & -0.020 \\
LSQ13aiz & -0.03 & 0.14 & 0.035 & 0.030 & 0.108 & 0.015 & -0.696 & 0.211 & -4.338 & 0.430 & -0.213 \\
LSQ13avx & 0.93 & 0.24 & 0.182 & 0.037 & 0.403 & 0.015 & 0.157 & 0.086 & 2.902 & 3.621 & 1.923 \\
LSQ13vy & -1.29 & 0.12 & 0.036 & 0.031 & 0.306 & 0.015 & -0.013 & 0.053 & -5.377 & 0.206 & -0.365 \\
LSQ14cnm & 0.25 & 0.16 & -0.088 & 0.029 & -0.231 & 0.012 & 0.013 & 0.067 & -0.907 & 1.532 & -0.317 \\
PTF09dlc & 0.34 & 0.14 & -0.065 & 0.029 & -0.187 & 0.012 & 0.082 & 0.035 & -1.321 & 1.747 & 0.675 \\
PTF09dnl & 0.92 & 0.12 & 0.064 & 0.027 & 0.013 & 0.012 & -0.100 & 0.094 & -2.311 & 0.990 & -1.515 \\
PTF09dnp & -0.53 & 0.24 & -0.042 & 0.030 & -0.082 & 0.012 & -0.140 & 0.059 & 2.393 & -1.621 & -2.697 \\
PTF09fox & 0.50 & 0.29 & -0.064 & 0.032 & -0.199 & 0.012 & 0.011 & 0.033 & -0.767 & 0.079 & -0.429 \\
PTF09foz & -0.95 & 0.32 & 0.001 & 0.034 & 0.033 & 0.012 & -0.042 & 0.042 & -0.843 & -0.410 & 2.067 \\
PTF10hmv & 1.35 & 0.16 & 0.144 & 0.031 & 0.353 & 0.012 & 0.131 & 0.068 & 0.912 & 1.498 & 1.473 \\
PTF10icb & 0.38 & 0.11 & 0.052 & 0.028 & 0.153 & 0.012 & 0.409 & 0.242 & 1.403 & -0.703 & 0.211 \\
PTF10mwb & -0.75 & 0.10 & -0.031 & 0.027 & 0.117 & 0.012 & 0.034 & 0.070 & 0.357 & -1.527 & 0.865 \\
PTF10ndc & 1.17 & 0.18 & -0.054 & 0.028 & -0.219 & 0.012 & 0.002 & 0.029 & -0.292 & 1.166 & -1.182 \\
PTF10nlg & 0.78 & 0.15 & 0.131 & 0.029 & 0.381 & 0.013 & 0.072 & 0.040 & -4.297 & 0.034 & 0.248 \\
PTF10qjl & 1.50 & 0.17 & -0.026 & 0.031 & -0.161 & 0.015 & 0.008 & 0.040 & -0.814 & 1.134 & 0.003 \\
PTF10qjq & -0.16 & 0.11 & 0.039 & 0.029 & 0.110 & 0.012 & -0.097 & 0.078 & 2.188 & -0.686 & -0.722 \\
PTF10qyz & -1.30 & 0.19 & -0.135 & 0.031 & -0.096 & 0.013 & 0.236 & 0.036 & -0.480 & -2.388 & 1.129 \\
PTF10tce & 0.60 & 0.14 & 0.054 & 0.029 & -0.048 & 0.013 & 0.017 & 0.056 & -3.169 & 1.311 & -0.444 \\
PTF10ufj & 0.11 & 0.16 & -0.109 & 0.030 & -0.129 & 0.013 & 0.055 & 0.032 & -1.383 & 0.824 & 1.659 \\
PTF10wnm & 0.65 & 0.15 & -0.020 & 0.029 & -0.114 & 0.012 & 0.021 & 0.035 & 0.716 & 0.934 & -1.147 \\
PTF10wof & 0.26 & 0.15 & 0.010 & 0.030 & 0.029 & 0.012 & 0.103 & 0.044 & -2.955 & -0.318 & 0.401 \\
PTF10ygu & 0.27 & 0.12 & 0.453 & 0.029 & 0.832 & 0.013 & -0.295 & 0.084 & -4.368 & 1.622 & -2.407 \\
PTF10zdk & 0.32 & 0.18 & 0.091 & 0.034 & 0.235 & 0.012 & 0.032 & 0.069 & -2.089 & 0.941 & 2.326 \\
PTF11bgv & -0.15 & 0.12 & 0.068 & 0.030 & 0.301 & 0.012 & -0.029 & 0.066 & 2.559 & -0.907 & -0.892 \\
PTF11bju & 1.02 & 0.18 & 0.042 & 0.032 & 0.035 & 0.012 & -0.165 & 0.066 & 4.963 & 1.169 & -0.704 \\
PTF11bnx & 0.01 & 0.17 & 0.106 & 0.032 & 0.243 & 0.013 & 0.126 & 0.041 & -2.134 & 0.108 & 1.520 \\
PTF11bui & 0.77 & 0.11 & 0.066 & 0.029 & 0.029 & 0.012 & 0.043 & 0.076 & -2.001 & 1.484 & -2.695 \\
PTF11cao & 0.17 & 0.15 & 0.060 & 0.031 & 0.193 & 0.012 & -0.045 & 0.055 & -3.671 & -0.405 & 0.992 \\
PTF11drz & 0.54 & 0.46 & 0.024 & 0.037 & 0.006 & 0.012 & 0.063 & 0.039 & -1.599 & -0.398 & 0.279 \\
PTF11kjn & -2.45 & 0.09 & 0.264 & 0.030 & 1.180 & 0.013 & -0.026 & 0.098 & -0.322 & -5.244 & 1.655 \\
PTF11kly & -0.62 & 0.09 & -0.074 & 0.026 & -0.131 & 0.012 & 0.632 & 1.799 & 1.425 & -1.163 & 0.373 \\
PTF11mkx & 0.73 & 0.16 & 0.035 & 0.030 & -0.006 & 0.012 & -0.483 & 0.042 & 5.172 & 1.258 & -0.701 \\
PTF11mty & 0.65 & 0.18 & -0.055 & 0.030 & -0.186 & 0.013 & -0.022 & 0.031 & 1.057 & 0.467 & -0.181 \\
PTF11pdk & 0.31 & 0.28 & -0.070 & 0.035 & -0.139 & 0.013 & 0.043 & 0.028 & 1.502 & -0.325 & 0.236 \\
PTF11qmo & 0.18 & 0.32 & -0.090 & 0.035 & -0.244 & 0.013 & -0.121 & 0.040 & 1.569 & 0.329 & 0.266 \\
PTF12ena & 0.90 & 0.14 & 0.308 & 0.031 & 0.753 & 0.012 & 0.029 & 0.126 & 0.667 & 0.911 & 0.517 \\
PTF12evo & 0.70 & 0.15 & 0.030 & 0.030 & 0.060 & 0.014 & -0.121 & 0.035 & -0.418 & 2.373 & 1.555 \\
PTF12fuu & 0.44 & 0.13 & -0.130 & 0.030 & -0.304 & 0.013 & 0.180 & 0.046 & 0.200 & 0.998 & -0.481 \\
PTF12ghy & -0.42 & 0.11 & 0.243 & 0.029 & 0.653 & 0.012 & -0.120 & 0.064 & 0.433 & -1.119 & 1.026 \\
PTF12grk & -1.54 & 0.15 & -0.046 & 0.031 & 0.152 & 0.014 & -0.027 & 0.034 & -5.189 & -0.108 & -0.010 \\
PTF12hwb & 0.76 & 0.14 & 0.182 & 0.029 & 0.339 & 0.017 & 0.152 & 0.043 & -2.235 & 1.899 & -1.791 \\
PTF12iiq & -1.23 & 0.11 & 0.009 & 0.028 & 0.139 & 0.013 & 0.074 & 0.077 & -6.109 & 0.178 & 0.090 \\
PTF12ikt & -0.20 & 0.12 & -0.032 & 0.029 & -0.029 & 0.012 & 0.020 & 0.050 & 1.742 & -1.218 & -0.432 \\
PTF12jqh & 1.00 & 0.19 & -0.034 & 0.031 & -0.194 & 0.013 & 0.076 & 0.048 & -1.892 & 1.761 & -1.271 \\
PTF13anh & -0.33 & 0.18 & -0.041 & 0.034 & -0.032 & 0.013 & 0.003 & 0.036 & -3.041 & -0.523 & 1.040 \\
PTF13asv & 0.49 & 0.10 & -0.151 & 0.027 & -0.440 & 0.012 & 0.087 & 0.064 & 2.922 & 0.213 & -1.197 \\
PTF13ayw & -1.48 & 0.28 & -0.038 & 0.037 & 0.092 & 0.013 & 0.089 & 0.042 & -0.625 & -2.126 & -1.118 \\
PTF13azs & 0.04 & 0.11 & 0.237 & 0.030 & 0.700 & 0.015 & 0.172 & 0.066 & -2.099 & -0.243 & 1.206 \\
SN2004ef & -1.32 & 0.25 & 0.074 & 0.031 & 0.294 & 0.012 & -0.036 & 0.074 & -3.369 & -0.565 & -0.575 \\
SN2004gc & -0.02 & 0.15 & 0.057 & 0.036 & 0.062 & 0.018 & -0.097 & 0.070 & -2.959 & -0.283 & 1.954 \\
SN2005M & 0.59 & 0.65 & 0.009 & 0.031 & 0.002 & 0.012 & -0.213 & 0.085 & 1.699 & 2.719 & 2.625 \\
SN2005cc & -1.17 & 0.20 & 0.383 & 0.038 & 1.275 & 0.015 & 1.405 & 0.277 & 4.995 & 3.982 & 2.611 \\
SN2005cf & -0.11 & 0.17 & -0.035 & 0.032 & -0.135 & 0.012 & 0.034 & 0.310 & -1.569 & 1.095 & 0.403 \\
SN2005cg & 1.26 & 0.33 & -0.055 & 0.034 & -0.233 & 0.013 & 0.078 & 0.072 & -1.215 & 1.585 & -0.468 \\
SN2005di & -0.61 & 0.20 & 0.357 & 0.034 & 1.100 & 0.013 & -0.003 & 0.090 & 1.254 & -1.050 & 0.655 \\
SN2005el & -1.30 & 0.10 & -0.175 & 0.030 & -0.144 & 0.014 & 0.106 & 0.146 & 0.543 & -0.748 & -0.974 \\
SN2005hc & 1.07 & 0.32 & -0.050 & 0.033 & -0.277 & 0.012 & 0.205 & 0.049 & -1.462 & 1.587 & -0.356 \\
SN2005hj & 1.63 & 0.40 & 0.014 & 0.035 & -0.092 & 0.013 & -0.130 & 0.040 & 3.195 & 0.350 & -0.857 \\
SN2005ir & 1.27 & 0.58 & 0.027 & 0.046 & -0.118 & 0.015 & -0.094 & 0.032 & -2.734 & 1.240 & -2.243 \\
SN2005ki & -1.43 & 0.64 & -0.102 & 0.039 & -0.092 & 0.012 & 0.018 & 0.105 & 0.216 & -1.920 & -0.936 \\
SN2006X & 0.34 & 0.20 & 1.246 & 0.039 & 3.315 & 0.019 & -2.088 & 0.344 & -6.338 & 2.749 & -1.139 \\
SN2006cj & 0.40 & 0.18 & -0.059 & 0.030 & -0.123 & 0.012 & 0.001 & 0.034 & 1.218 & 0.386 & -0.931 \\
SN2006dm & -1.88 & 0.33 & -0.033 & 0.036 & 0.236 & 0.012 & 0.087 & 0.105 & -0.866 & -2.929 & 0.763 \\
SN2006do & -1.91 & 0.45 & -0.027 & 0.035 & 0.165 & 0.012 & -0.029 & 0.080 & -1.950 & -0.992 & -0.807 \\
SN2006ob & -2.43 & 0.32 & -0.051 & 0.036 & 0.123 & 0.012 & 0.013 & 0.039 & 0.051 & -2.752 & -0.438 \\
SN2007bc & -0.74 & 0.29 & -0.008 & 0.037 & -0.027 & 0.017 & 0.047 & 0.100 & 2.087 & -1.630 & 0.096 \\
SN2007bd & -0.65 & 0.33 & -0.081 & 0.031 & -0.092 & 0.012 & 0.045 & 0.070 & -1.008 & -0.829 & -0.773 \\
SN2007cq & -0.34 & 0.16 & -0.076 & 0.031 & -0.080 & 0.013 & -0.168 & 0.088 & 2.347 & -1.314 & 0.048 \\
SN2007fr & -2.62 & 0.12 & -0.019 & 0.031 & 0.406 & 0.013 & 0.031 & 0.045 & 0.492 & -3.858 & 0.265 \\
SN2007kk & 0.85 & 0.21 & -0.009 & 0.030 & -0.140 & 0.012 & -0.208 & 0.054 & -2.511 & 1.594 & -0.989 \\
SN2007le & 0.46 & 0.19 & 0.270 & 0.033 & 0.613 & 0.013 & 0.263 & 0.393 & -3.651 & 0.689 & -0.291 \\
SN2007nq & -2.16 & 0.35 & -0.029 & 0.041 & 0.142 & 0.013 & -0.059 & 0.051 & -1.522 & -2.520 & 0.262 \\
SN2007qe & 0.86 & 0.29 & 0.068 & 0.039 & 0.076 & 0.013 & 0.069 & 0.096 & -5.130 & 0.692 & -0.246 \\
SN2008ec & -1.05 & 0.11 & 0.107 & 0.029 & 0.414 & 0.012 & -0.044 & 0.145 & 0.349 & -1.878 & 0.285 \\
SN2009hi & -2.14 & 0.10 & 0.097 & 0.037 & 0.581 & 0.017 & -0.030 & 0.056 & -1.037 & -2.781 & -1.823 \\
SN2009hs & -2.59 & 0.12 & 0.100 & 0.032 & 0.676 & 0.012 & 0.140 & 0.079 & 1.631 & -4.466 & 0.586 \\
SN2009ig & 0.98 & 0.05 & 0.004 & 0.025 & -0.065 & 0.012 & -0.095 & 0.271 & -1.942 & 1.601 & -2.451 \\
SN2010dt & 0.04 & 0.12 & -0.074 & 0.029 & -0.113 & 0.012 & 0.021 & 0.042 & -0.373 & -1.512 & 1.330 \\
SN2010ex & 0.54 & 0.15 & -0.074 & 0.029 & -0.193 & 0.012 & 0.251 & 0.101 & -0.085 & 0.766 & -0.393 \\
SN2010kg & -1.45 & 0.65 & 0.077 & 0.039 & 0.320 & 0.012 & -0.158 & 0.135 & -4.318 & 1.297 & -2.108 \\
SN2011ay & -1.10 & 0.18 & 0.453 & 0.035 & 1.137 & 0.012 & -0.527 & 0.103 & 6.457 & 4.892 & 2.832 \\
SN2012cu & 0.19 & 0.10 & 1.036 & 0.031 & 2.772 & 0.012 & -0.216 & 0.475 & 1.857 & 0.035 & -0.258 \\
SN2012fr & 0.92 & 0.08 & -0.054 & 0.027 & -0.272 & 0.012 & -0.369 & 0.423 & -2.216 & 2.008 & -1.701 \\
SNBOSS38 & 1.44 & 0.09 & 0.146 & 0.028 & 0.321 & 0.011 & -0.282 & 0.230 & 2.548 & -2.252 & -1.761 \\
SNF20050728-006 & 0.46 & 0.31 & 0.117 & 0.035 & 0.276 & 0.014 & -0.094 & 0.039 & -0.937 & -0.557 & 0.339 \\
SNF20050729-002 & 0.92 & 0.34 & -0.107 & 0.038 & -0.260 & 0.018 & 0.128 & 0.030 & 0.621 & -0.536 & 0.152 \\
SNF20050821-007 & 0.42 & 0.29 & -0.043 & 0.036 & -0.205 & 0.014 & 0.029 & 0.040 & -2.580 & 2.821 & 0.355 \\
SNF20050927-005 & 0.19 & 0.35 & 0.018 & 0.035 & 0.033 & 0.014 & 0.301 & 0.056 & -0.176 & -1.688 & 1.221 \\
SNF20051003-004 & 1.16 & 0.16 & -0.100 & 0.030 & -0.349 & 0.013 & 0.071 & 0.065 & 2.030 & 0.489 & -1.463 \\
SNF20060511-014 & -0.78 & 0.18 & -0.041 & 0.035 & -0.030 & 0.013 & 0.037 & 0.048 & -0.396 & -1.828 & 1.501 \\
SNF20060512-001 & 0.40 & 0.14 & -0.007 & 0.030 & 0.046 & 0.012 & -0.096 & 0.057 & 1.810 & 2.584 & 2.179 \\
SNF20060512-002 & -0.26 & 0.23 & 0.086 & 0.033 & 0.079 & 0.015 & -0.197 & 0.045 & -1.993 & 1.080 & -1.411 \\
SNF20060521-001 & -1.63 & 0.29 & -0.111 & 0.036 & -0.057 & 0.013 & 0.047 & 0.034 & 1.238 & -2.242 & -0.497 \\
SNF20060521-008 & -1.35 & 0.32 & 0.122 & 0.042 & 0.404 & 0.016 & -0.206 & 0.041 & -3.916 & -0.466 & -1.604 \\
SNF20060526-003 & 0.30 & 0.25 & -0.018 & 0.031 & -0.051 & 0.013 & -0.027 & 0.030 & -0.224 & 0.762 & -0.465 \\
SNF20060530-003 & 1.37 & 0.20 & -0.042 & 0.031 & -0.268 & 0.017 & -0.057 & 0.041 & -1.368 & 1.565 & -2.242 \\
SNF20060609-002 & 0.27 & 0.15 & 0.206 & 0.031 & 0.547 & 0.013 & -0.153 & 0.056 & 2.366 & -0.055 & -1.155 \\
SNF20060618-023 & -0.12 & 0.19 & 0.046 & 0.032 & 0.030 & 0.017 & -0.267 & 0.026 & 3.413 & 1.145 & 0.343 \\
SNF20060621-015 & 0.51 & 0.22 & -0.102 & 0.031 & -0.247 & 0.012 & -0.031 & 0.041 & 0.863 & 0.107 & 0.712 \\
SNF20060907-000 & -0.12 & 0.22 & -0.108 & 0.030 & -0.214 & 0.012 & 0.084 & 0.040 & 0.315 & -0.928 & 1.679 \\
SNF20060908-004 & 0.74 & 0.17 & -0.040 & 0.030 & -0.175 & 0.014 & -0.088 & 0.046 & -0.809 & 2.231 & 0.996 \\
SNF20060911-014 & 0.51 & 0.16 & -0.179 & 0.027 & -0.435 & 0.013 & 0.160 & 0.026 & 1.525 & 0.978 & -2.005 \\
SNF20060912-000 & 0.16 & 0.21 & 0.109 & 0.030 & 0.288 & 0.014 & -0.314 & 0.033 & -0.566 & 1.326 & 3.064 \\
SNF20060916-002 & 1.59 & 0.27 & -0.036 & 0.035 & -0.170 & 0.015 & -0.066 & 0.033 & 0.929 & 0.772 & -1.209 \\
SNF20061011-005 & 0.72 & 0.24 & -0.149 & 0.034 & -0.278 & 0.015 & -0.080 & 0.097 & 0.096 & 0.788 & -0.668 \\
SNF20061020-000 & -1.89 & 0.20 & -0.014 & 0.034 & 0.161 & 0.012 & 0.023 & 0.058 & -0.259 & -2.830 & 0.122 \\
SNF20061021-003 & 0.09 & 0.18 & 0.041 & 0.031 & 0.147 & 0.013 & -0.099 & 0.037 & -0.005 & -0.083 & 0.337 \\
SNF20061022-005 & 1.02 & 0.24 & 0.048 & 0.031 & 0.000 & 0.013 & -0.106 & 0.030 & 4.215 & 0.716 & -1.031 \\
SNF20061024-000 & -1.88 & 0.17 & -0.062 & 0.033 & 0.131 & 0.014 & 0.072 & 0.041 & -0.639 & -2.885 & 0.628 \\
SNF20061030-010 & 0.26 & 0.22 & 0.118 & 0.032 & 0.244 & 0.013 & 0.076 & 0.079 & -2.686 & 0.193 & 0.011 \\
SNF20061111-002 & 0.30 & 0.23 & -0.021 & 0.032 & -0.025 & 0.013 & 0.057 & 0.034 & -0.386 & -1.718 & 1.437 \\
SNF20070330-024 & 0.70 & 0.26 & -0.096 & 0.031 & -0.295 & 0.013 & -0.147 & 0.053 & -1.074 & 1.215 & -1.875 \\
SNF20070403-001 & -0.52 & 0.14 & -0.009 & 0.029 & 0.018 & 0.014 & -0.063 & 0.030 & -0.128 & -1.839 & 0.792 \\
SNF20070424-003 & 0.43 & 0.11 & -0.031 & 0.030 & 0.012 & 0.018 & -0.028 & 0.037 & -1.838 & 0.526 & 0.638 \\
SNF20070427-001 & 0.92 & 0.20 & -0.113 & 0.032 & -0.327 & 0.013 & -0.080 & 0.030 & 3.543 & -0.550 & -1.397 \\
SNF20070506-006 & 1.25 & 0.12 & -0.058 & 0.029 & -0.173 & 0.012 & -0.146 & 0.062 & 2.001 & 1.803 & 0.867 \\
SNF20070528-003 & 1.29 & 0.25 & 0.083 & 0.034 & 0.017 & 0.015 & -0.587 & 0.023 & 6.096 & 1.262 & -1.347 \\
SNF20070531-011 & -1.58 & 0.19 & -0.072 & 0.031 & 0.058 & 0.012 & -0.034 & 0.061 & -1.189 & -1.771 & -0.120 \\
SNF20070630-006 & 0.42 & 0.12 & 0.008 & 0.030 & -0.026 & 0.014 & -0.084 & 0.033 & -1.396 & 0.342 & 0.087 \\
SNF20070701-005 & -0.05 & 0.16 & 0.009 & 0.031 & -0.011 & 0.014 & -0.255 & 0.034 & 0.523 & 2.056 & 2.914 \\
SNF20070712-000 & 0.03 & 0.21 & -0.044 & 0.032 & -0.060 & 0.016 & 0.031 & 0.074 & 0.406 & -1.215 & -0.016 \\
SNF20070712-003 & 0.05 & 0.19 & -0.129 & 0.032 & -0.189 & 0.013 & 0.039 & 0.032 & 1.206 & -1.116 & 0.867 \\
SNF20070725-001 & 0.66 & 0.16 & -0.136 & 0.031 & -0.251 & 0.014 & 0.001 & 0.035 & 0.618 & 0.708 & 0.265 \\
SNF20070727-016 & 0.46 & 0.14 & -0.083 & 0.030 & -0.222 & 0.013 & -0.229 & 0.035 & 3.383 & 0.384 & -1.037 \\
SNF20070802-000 & 0.32 & 0.17 & 0.110 & 0.031 & 0.139 & 0.014 & -0.057 & 0.036 & -4.055 & 0.428 & -0.272 \\
SNF20070803-005 & 0.89 & 0.17 & -0.004 & 0.030 & -0.159 & 0.013 & -0.295 & 0.072 & 5.268 & 1.261 & -0.795 \\
SNF20070806-026 & -1.90 & 0.13 & -0.099 & 0.032 & 0.052 & 0.013 & 0.038 & 0.050 & -0.221 & -2.493 & -0.334 \\
SNF20070810-004 & 0.16 & 0.15 & -0.028 & 0.030 & -0.025 & 0.014 & -0.014 & 0.029 & -2.309 & -1.200 & 0.521 \\
SNF20070817-003 & -0.66 & 0.14 & -0.124 & 0.029 & -0.086 & 0.014 & 0.099 & 0.034 & -1.073 & -1.267 & 0.230 \\
SNF20070831-015 & 1.69 & 0.20 & 0.031 & 0.031 & -0.096 & 0.013 & -0.090 & 0.034 & 0.264 & 2.600 & 1.466 \\
SNF20070902-018 & -0.53 & 0.11 & 0.055 & 0.029 & 0.230 & 0.014 & -0.009 & 0.034 & -0.186 & -1.972 & 0.805 \\
SNF20070902-021 & -0.30 & 0.12 & -0.018 & 0.030 & 0.000 & 0.014 & -0.074 & 0.032 & 0.970 & -1.833 & 0.303 \\
SNF20070912-000 & 0.30 & 0.27 & 0.053 & 0.035 & -0.051 & 0.019 & -0.396 & 0.027 & 4.885 & 2.291 & 1.005 \\
SNF20071015-000 & 0.70 & 0.22 & 0.359 & 0.032 & 0.874 & 0.013 & 0.031 & 0.059 & 1.387 & 0.073 & -0.799 \\
SNF20071021-000 & -0.46 & 0.21 & 0.039 & 0.031 & 0.159 & 0.012 & 0.038 & 0.083 & -4.187 & 0.039 & 0.772 \\
SNF20071108-021 & 0.93 & 0.29 & -0.065 & 0.031 & -0.196 & 0.013 & -0.141 & 0.031 & 1.390 & 2.470 & 1.102 \\
SNF20080323-009 & 0.54 & 0.15 & -0.069 & 0.030 & -0.248 & 0.014 & 0.033 & 0.029 & 3.150 & -0.999 & -1.450 \\
SNF20080507-000 & 0.86 & 0.22 & 0.078 & 0.031 & 0.100 & 0.013 & -0.196 & 0.042 & 0.494 & 2.456 & 1.543 \\
SNF20080510-001 & 0.37 & 0.19 & -0.077 & 0.031 & -0.144 & 0.013 & 0.042 & 0.032 & -0.733 & -1.175 & 0.491 \\
SNF20080510-005 & 1.08 & 0.22 & -0.054 & 0.031 & -0.147 & 0.014 & 0.020 & 0.028 & -0.349 & 0.832 & -1.333 \\
SNF20080512-008 & 1.15 & 0.18 & -0.050 & 0.032 & -0.278 & 0.017 & 0.001 & 0.032 & -0.996 & 2.055 & -0.562 \\
SNF20080512-010 & -1.53 & 0.26 & -0.064 & 0.033 & 0.019 & 0.013 & -0.011 & 0.036 & 0.046 & -1.928 & -1.315 \\
SNF20080514-002 & -1.70 & 0.11 & -0.129 & 0.028 & -0.119 & 0.012 & 0.265 & 0.095 & 1.583 & -1.987 & -0.211 \\
SNF20080516-000 & 1.31 & 0.22 & -0.064 & 0.032 & -0.247 & 0.014 & 0.059 & 0.032 & -0.022 & 1.871 & 0.043 \\
SNF20080516-022 & 0.05 & 0.14 & -0.098 & 0.029 & -0.178 & 0.013 & -0.003 & 0.031 & 2.414 & -0.716 & 0.044 \\
SNF20080522-000 & 1.18 & 0.13 & -0.022 & 0.029 & -0.125 & 0.012 & -0.238 & 0.048 & 4.274 & 0.877 & -0.619 \\
SNF20080522-011 & 0.92 & 0.18 & -0.072 & 0.030 & -0.216 & 0.012 & -0.117 & 0.058 & -0.239 & 0.135 & -0.134 \\
SNF20080531-000 & -0.36 & 0.20 & -0.040 & 0.031 & -0.066 & 0.012 & 0.119 & 0.060 & -1.980 & -0.642 & 1.113 \\
SNF20080610-000 & 0.31 & 0.19 & -0.041 & 0.031 & -0.001 & 0.014 & 0.041 & 0.031 & -0.345 & -1.526 & 1.451 \\
SNF20080612-003 & 0.81 & 0.20 & -0.036 & 0.030 & -0.080 & 0.012 & -0.318 & 0.067 & -0.471 & 1.037 & -0.800 \\
SNF20080614-010 & -1.86 & 0.19 & -0.027 & 0.034 & 0.212 & 0.015 & -0.008 & 0.033 & 0.451 & -2.540 & -0.647 \\
SNF20080620-000 & -0.92 & 0.16 & 0.012 & 0.031 & 0.145 & 0.012 & 0.086 & 0.066 & -0.772 & -1.466 & 1.251 \\
SNF20080623-001 & -0.01 & 0.14 & -0.062 & 0.029 & -0.126 & 0.012 & 0.162 & 0.050 & -1.908 & -0.565 & 1.183 \\
SNF20080626-002 & 1.13 & 0.21 & -0.043 & 0.030 & -0.161 & 0.012 & -0.061 & 0.093 & -1.147 & 1.210 & -1.560 \\
SNF20080717-000 & 0.48 & 0.12 & 0.175 & 0.029 & 0.425 & 0.013 & -0.110 & 0.039 & -0.431 & 1.126 & -2.016 \\
SNF20080720-001 & 0.13 & 0.11 & 0.390 & 0.027 & 1.013 & 0.012 & -0.177 & 0.110 & -2.419 & 1.827 & -0.509 \\
SNF20080723-012 & 0.73 & 0.12 & 0.004 & 0.029 & -0.106 & 0.013 & -0.461 & 0.031 & 4.752 & 1.097 & -0.663 \\
SNF20080725-004 & 0.99 & 0.16 & 0.005 & 0.030 & -0.035 & 0.013 & 0.074 & 0.042 & -1.582 & 2.443 & 0.603 \\
SNF20080803-000 & 0.58 & 0.14 & 0.112 & 0.031 & 0.195 & 0.014 & -0.018 & 0.040 & -0.824 & 0.675 & -0.401 \\
SNF20080806-002 & 1.09 & 0.18 & 0.049 & 0.031 & 0.023 & 0.013 & -0.070 & 0.037 & -0.888 & 1.708 & -0.141 \\
SNF20080810-001 & -0.98 & 0.12 & -0.022 & 0.029 & 0.083 & 0.012 & -0.000 & 0.052 & 1.881 & -1.738 & 0.175 \\
SNF20080821-000 & 0.45 & 0.17 & 0.013 & 0.029 & 0.013 & 0.013 & -0.127 & 0.032 & -0.010 & 0.542 & -1.024 \\
SNF20080822-005 & 0.75 & 0.21 & -0.051 & 0.031 & -0.178 & 0.013 & -0.140 & 0.033 & 2.956 & 0.532 & -0.389 \\
SNF20080825-010 & -0.84 & 0.18 & -0.028 & 0.031 & -0.015 & 0.012 & -0.141 & 0.055 & -0.227 & -1.883 & 0.224 \\
SNF20080905-005 & -1.84 & 0.25 & 0.139 & 0.039 & 0.598 & 0.012 & -0.502 & 0.040 & 0.886 & -3.446 & -1.355 \\
SNF20080908-000 & 0.29 & 0.19 & -0.100 & 0.031 & -0.176 & 0.017 & -0.074 & 0.046 & -1.467 & 0.581 & 1.375 \\
SNF20080909-030 & 1.25 & 0.14 & 0.007 & 0.029 & -0.040 & 0.012 & -0.094 & 0.073 & 1.548 & 2.379 & 2.116 \\
SNF20080913-031 & 0.19 & 0.20 & 0.040 & 0.034 & 0.077 & 0.013 & -0.102 & 0.041 & -0.735 & 1.344 & 3.551 \\
SNF20080914-001 & -0.10 & 0.14 & 0.132 & 0.031 & 0.402 & 0.012 & -0.120 & 0.093 & 0.051 & 0.837 & 1.875 \\
SNF20080918-000 & 1.47 & 0.28 & 0.155 & 0.036 & 0.197 & 0.013 & 0.042 & 0.035 & -2.033 & 2.237 & -0.926 \\
SNF20080918-002 & -0.32 & 0.12 & -0.048 & 0.029 & -0.111 & 0.014 & 0.071 & 0.029 & 2.077 & -1.277 & 0.018 \\
SNF20080918-004 & -1.18 & 0.19 & -0.083 & 0.032 & -0.007 & 0.013 & 0.228 & 0.045 & -0.191 & -2.082 & 1.048 \\
SNF20080919-000 & 0.21 & 0.15 & 0.189 & 0.031 & 0.499 & 0.013 & -0.026 & 0.039 & 0.239 & 1.010 & -0.569 \\
SNF20080919-001 & 0.94 & 0.17 & 0.000 & 0.031 & -0.019 & 0.012 & -0.390 & 0.054 & 2.132 & 1.694 & 2.067 \\
SNF20080919-002 & -1.42 & 0.16 & 0.000 & 0.034 & 0.343 & 0.016 & 0.099 & 0.042 & 0.396 & -3.144 & 0.430 \\
SNF20080920-000 & 1.26 & 0.27 & 0.011 & 0.032 & -0.174 & 0.013 & 0.000 & 0.056 & -2.277 & 1.567 & -2.006 \\
SNF20080926-009 & 0.42 & 0.15 & 0.008 & 0.031 & -0.078 & 0.014 & -0.121 & 0.033 & -0.499 & 0.586 & 3.121 \\
SN2013be & 0.56 & 0.19 & 0.047 & 0.034 & 0.072 & 0.013 & -0.223 & 0.034 & -0.263 & 1.608 & 2.769 \\
PSNJ02263653+1208555 & 0.73 & 0.13 & 0.097 & 0.029 & 0.135 & 0.012 & 0.006 & 0.082 & -3.500 & 1.090 & -0.504 \\
SNNGC2691 & 1.00 & 0.18 & 0.080 & 0.032 & 0.128 & 0.012 & -0.249 & 0.156 & 4.671 & 1.023 & -0.739 \\
SN2011bc & -0.07 & 0.10 & 0.101 & 0.028 & 0.278 & 0.012 & -0.052 & 0.100 & -0.674 & 2.468 & 1.920 \\
SNNGC4424 & 0.48 & 0.11 & 0.092 & 0.029 & 0.211 & 0.012 & 0.605 & 0.843 & 0.820 & 0.881 & 0.102 \\
SN2013bs & -2.21 & 0.23 & -0.039 & 0.035 & 0.278 & 0.012 & 0.027 & 0.080 & 0.543 & -3.767 & 1.164 \\
SNNGC6430 & -2.73 & 0.12 & 0.313 & 0.033 & 1.203 & 0.013 & 0.183 & 0.218 & -3.135 & -4.358 & 1.985 \\
PSNJ20435314+1230304 & -2.03 & 0.38 & 0.161 & 0.037 & 0.792 & 0.012 & 0.125 & 0.150 & -1.162 & -3.760 & 1.478 \\
SNPGC027923 & 0.46 & 0.26 & -0.172 & 0.032 & -0.393 & 0.012 & 0.068 & 0.120 & 2.838 & -0.238 & -1.809 \\
SN2013bt & -1.95 & 0.17 & -0.113 & 0.033 & 0.019 & 0.012 & 0.037 & 0.060 & 0.656 & -1.978 & -1.060 \\
SN2015N & 0.51 & 0.58 & 0.084 & 0.038 & 0.073 & 0.012 & -0.911 & 0.123 & -4.022 & 1.417 & -2.174 \\
SNUGC2855 & -0.28 & 0.16 & -0.097 & 0.031 & -0.231 & 0.012 & 0.046 & 0.585 & 2.628 & -0.183 & -1.629 \\
AT2015bp & -2.44 & 0.21 & -0.058 & 0.035 & 0.285 & 0.012 & 0.922 & 0.461 & 0.761 & -3.361 & 0.518 \\
SN2011be & 0.48 & 0.23 & -0.071 & 0.032 & -0.161 & 0.012 & 0.096 & 0.062 & 2.175 & -0.609 & -0.956 \\
SN2011ho & -1.78 & 0.19 & 0.035 & 0.039 & 0.413 & 0.013 & 0.211 & 0.067 & -0.886 & -3.588 & 0.063 \\


==> snfactory_authorlist.tex <==
\author[0000-0002-5828-6211]{K.~Boone}
\affiliation{Physics Division, Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA, 94720, USA}
\affiliation{Department of Physics, University of California Berkeley, 366 LeConte Hall MC 7300, Berkeley, CA, 94720-7300, USA}
\affiliation{DIRAC Institute, Department of Astronomy, University of Washington, 3910 15th Ave NE, Seattle, WA, 98195, USA}

\author{G.~Aldering}
\affiliation{Physics Division, Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA, 94720, USA}

\author[0000-0002-0389-5706]{P.~Antilogus}
\affiliation{Laboratoire de Physique Nucl\'eaire et des Hautes Energies, CNRS/IN2P3, Sorbonne Universit\'e, Universit\'e de Paris, 4 place Jussieu, 75005 Paris, France}

\author[0000-0002-9502-0965]{C.~Aragon}
\affiliation{Physics Division, Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA, 94720, USA}
\affiliation{College of Engineering, University of Washington 371 Loew Hall, Seattle, WA, 98195, USA}

\author{S.~Bailey}
\affiliation{Physics Division, Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA, 94720, USA}

\author[0000-0003-0424-8719]{C.~Baltay}
\affiliation{Department of Physics, Yale University, New Haven, CT, 06250-8121, USA}

\author{S.~Bongard}
\affiliation{Laboratoire de Physique Nucl\'eaire et des Hautes Energies, CNRS/IN2P3, Sorbonne Universit\'e, Universit\'e de Paris, 4 place Jussieu, 75005 Paris, France}

\author[0000-0002-3780-7516]{C.~Buton}
\affiliation{Univ Lyon, Univ Claude Bernard Lyon~1, CNRS, IP2I~Lyon / IN2P3, UMR~5822, F-69622, Villeurbanne, France}
    
\author[0000-0002-5317-7518]{Y.~Copin}
\affiliation{Univ Lyon, Univ Claude Bernard Lyon~1, CNRS, IP2I~Lyon / IN2P3, UMR~5822, F-69622, Villeurbanne, France}

\author[0000-0003-1861-0870]{S.~Dixon}
\affiliation{Physics Division, Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA, 94720, USA}
\affiliation{Department of Physics, University of California Berkeley, 366 LeConte Hall MC 7300, Berkeley, CA, 94720-7300, USA}

\author[0000-0002-7496-3796]{D.~Fouchez}
\affiliation{Aix Marseille Univ, CNRS/IN2P3, CPPM, Marseille, France}

\author[0000-0001-6728-1423]{E.~Gangler}  
\affiliation{Univ Lyon, Univ Claude Bernard Lyon~1, CNRS, IP2I~Lyon / IN2P3, UMR~5822, F-69622, Villeurbanne, France}
\affiliation{Universit\'e Clermont Auvergne, CNRS/IN2P3, Laboratoire de Physique de Clermont, F-63000 Clermont-Ferrand, France}

\author[0000-0003-1820-4696]{R.~Gupta}
\affiliation{Physics Division, Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA, 94720, USA}

\author[0000-0001-9200-8699]{B.~Hayden}
\affiliation{Physics Division, Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA, 94720, USA}
\affiliation{Space Telescope Science Institute, 3700 San Martin Drive Baltimore, MD, 21218, USA}

\author{W.~Hillebrandt}
\affiliation{Max-Planck-Institut f\"ur Astrophysik,  Karl-Schwarzschild-Str. 1, D-85748 Garching, Germany}

\author[0000-0001-6315-8743]{A.~G.~Kim}
\affiliation{Physics Division, Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA, 94720, USA}

\author[0000-0001-8594-8666]{M.~Kowalski}
\affiliation{Institut f\"ur Physik,  Humboldt-Universitat zu Berlin, Newtonstr. 15, 12489 Berlin, Germany}
\affiliation {DESY, D-15735 Zeuthen, Germany}

\author{D.~K\"usters}
\affiliation {Department of Physics, University of California Berkeley, 366 LeConte Hall MC 7300, Berkeley, CA, 94720-7300, USA}
\affiliation {DESY, D-15735 Zeuthen, Germany}


\author[0000-0002-8357-3984]{P.-F.~L\'eget}
\affiliation{Laboratoire de Physique Nucl\'eaire et des Hautes Energies, CNRS/IN2P3, Sorbonne Universit\'e, Universit\'e de Paris, 4 place Jussieu, 75005 Paris, France}

\author{F.~Mondon}  
\affiliation{Universit\'e Clermont Auvergne, CNRS/IN2P3, Laboratoire de Physique de Clermont, F-63000 Clermont-Ferrand, France}

\author[0000-0001-8342-6274]{J.~Nordin}
\affiliation{Physics Division, Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA, 94720, USA}
\affiliation{Institut f\"ur Physik,  Humboldt-Universitat zu Berlin, Newtonstr. 15, 12489 Berlin, Germany}

\author[0000-0003-4016-6067]{R.~Pain}
\affiliation{Laboratoire de Physique Nucl\'eaire et des Hautes Energies, CNRS/IN2P3, Sorbonne Universit\'e, Universit\'e de Paris, 4 place Jussieu, 75005 Paris, France}

\author{E.~Pecontal}
\affiliation{Centre de Recherche Astronomique de Lyon, Universit\'e Lyon 1, 9 Avenue Charles Andr\'e, 69561 Saint Genis Laval Cedex, France}

\author{R.~Pereira}
\affiliation{Univ Lyon, Univ Claude Bernard Lyon~1, CNRS, IP2I~Lyon / IN2P3, UMR~5822, F-69622, Villeurbanne, France}

\author[0000-0002-4436-4661]{S.~Perlmutter}
\affiliation{Physics Division, Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA, 94720, USA}
\affiliation{Department of Physics, University of California Berkeley, 366 LeConte Hall MC 7300, Berkeley, CA, 94720-7300, USA}

\author[0000-0002-8207-3304]{K.~A.~Ponder}
\affiliation{Department of Physics, University of California Berkeley, 366 LeConte Hall MC 7300, Berkeley, CA, 94720-7300, USA}

\author{D.~Rabinowitz}
\affiliation{Department of Physics, Yale University, New Haven, CT, 06250-8121, USA}

 \author[0000-0002-8121-2560]{M.~Rigault} 
\affiliation{Institut f\"ur Physik,  Humboldt-Universitat zu Berlin, Newtonstr. 15, 12489 Berlin, Germany}
\affiliation{Univ Lyon, Univ Claude Bernard Lyon~1, CNRS, IP2I~Lyon / IN2P3, UMR~5822, F-69622, Villeurbanne, France}

\author[0000-0001-5402-4647]{D.~Rubin}
\affiliation{Physics Division, Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA, 94720, USA}
\affiliation{Department of Physics, University of Hawaii, 2505 Correa Rd, Honolulu, HI, 96822, USA}

\author{K.~Runge}
\affiliation{Physics Division, Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA, 94720, USA}

\author[0000-0002-4094-2102]{C.~Saunders}
\affiliation{Physics Division, Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA, 94720, USA}
\affiliation{Department of Physics, University of California Berkeley, 366 LeConte Hall MC 7300, Berkeley, CA, 94720-7300, USA}
\affiliation{Princeton University, Department of Astrophysics, 4 Ivy Lane, Princeton, NJ, 08544, USA}
\affiliation{Sorbonne Universit\'es, Institut Lagrange de Paris (ILP), 98 bis Boulevard Arago, 75014 Paris, France}

\author[0000-0002-9093-8849]{G.~Smadja}
\affiliation{Univ Lyon, Univ Claude Bernard Lyon~1, CNRS, IP2I~Lyon / IN2P3, UMR~5822, F-69622, Villeurbanne, France}

\author{N.~Suzuki}
\affiliation{Physics Division, Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA, 94720, USA}
\affiliation{Kavli Institute for the Physics and Mathematics of the Universe (WPI), The University of Tokyo Institutes for Advanced Study, The University of Tokyo, 5-1-5 Kashiwanoha, Kashiwa, Chiba 277-8583, Japan}

\author{C.~Tao}
\affiliation{Tsinghua Center for Astrophysics, Tsinghua University, Beijing 100084, China}
\affiliation{Aix Marseille Univ, CNRS/IN2P3, CPPM, Marseille, France}

\author[0000-0002-4265-1958]{S.~Taubenberger}
\affiliation{Max-Planck-Institut f\"ur Astrophysik, Karl-Schwarzschild-Str. 1, D-85748 Garching, Germany}

\author{R.~C.~Thomas}
\affiliation{Physics Division, Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA, 94720, USA}
\affiliation{Computational Cosmology Center, Computational Research Division, Lawrence Berkeley National Laboratory, 1 Cyclotron Road MS 50B-4206, Berkeley, CA, 94720, USA}

\author{M.~Vincenzi}
\affiliation{Physics Division, Lawrence Berkeley National Laboratory, 1 Cyclotron Road, Berkeley, CA, 94720, USA}
\affiliation{Institute of Cosmology and Gravitation, University of Portsmouth, Portsmouth, PO1 3FX, UK}

\collaboration{50}{The Nearby Supernova Factory}
